Relative representations enable zero-shot latent space communication

Neural networks embed the geometric structure of a data manifold lying in a high-dimensional space into latent representations. Ideally, the distribution of the data points in the latent space should depend only on the task, the data, the loss, and other architecture-specific constraints. However, factors such as the random weights initialization, training hyperparameters, or other sources of randomness in the training phase may induce incoherent latent spaces that hinder any form of reuse. Nevertheless, we empirically observe that, under the same data and modeling choices, the angles between the encodings within distinct latent spaces do not change. In this work, we propose the latent similarity between each sample and a fixed set of anchors as an alternative data representation, demonstrating that it can enforce the desired invariances without any additional training. We show how neural architectures can leverage these relative representations to guarantee, in practice, invariance to latent isometries and rescalings, effectively enabling latent space communication: from zero-shot model stitching to latent space comparison between diverse settings. We extensively validate the generalization capability of our approach on different datasets, spanning various modalities (images, text, graphs), tasks (e.g., classification, reconstruction) and architectures (e.g., CNNs, GCNs, transformers).

==> sections/dropped.tex <==
\subsection{Subspaces}\label{sec:subspaces}
This work does not assume the training data type, domain, or complexity, the embedding function $E$, or the downstream task to solve.
Nevertheless, the data Neural Networks deal with is often complex and presents intricate interactions.
Even when the function $E$ is learned end-to-end, in some cases a single scalar $r = sim(\ve_{\vx^{(i)}}, \ve_{\va^{(j)}})$ is not enough to meaningfully express the relationship between the sample $\vx^{(i)}$ and the anchor $\va^{(j)}$.

To address these complex settings, we propose a multidimensional representation for the similarity measure  $r = sim(\ve_{\vx^{(i)}}, \ve_{\va^{(j)}})$: we subdivide the absolute representations $\ve$ of the samples and the anchors in $\sS = \{1, \dots, s\}$ subspaces with size $l = \left\lfloor\dfrac{d}{s}\right\rfloor$. 
The absolute representation of the $j$ subspace is a contiguous portion of the original embedding $\ve^j = \ve_{(j-1) l : jl} \text{ with } j \in \sS$.
After that, we compute the subspaces relative representation independently:
$$
\vr^j_{\vx^{(i)}} = 
(
sim(\ve^j_{\vx^{(i)}}, \ve^j_{\va^{(1)}}),
sim(\ve^j_{\vx^{(i)}}, \ve^j_{\va^{(2)}}),
\dots,
sim(\ve^j_{\vx^{(i)}}, \ve^j_{\va^{(|\sA|)}})
) 
\text{ with } j \in \sS
$$

Projecting the data on independent subspaces, enable us to obtain more expressive relative representations and to distinguish more cases than considering the whole space. We show this behavior in the toy example in \cref{fig:subspace}
We define the relative representation of $\vx^{(i)}$ as the concatenation of the representation of each subspace:
$$
\vr^{\sS}_{\vx^{(i)}} = (\vr^1_{\vx^{(i)}}, \dots, \vr^s_{\vx^{(i)}})
$$
This formulation describes the similarity measure between a sample and each anchor with $s$ scalar numbers, 
enabling the modeling of complex data relationships.  We demonstrate the effectiveness of this strategy in \Cref{sec:subspace-comparison}.

\begin{figure}
    \centering
    \includegraphics[trim={0cm 8cm 0 0},width=\linewidth]{figures/p2.png}
    \caption{Consider two sets of points (in red and green respectively) lying on two different great circles on a sphere (top left). Taking the inner product between these sets of points (bottom left) give us limited information on their spatial distribution on the sphere. Instead if we project the points on the three subspaces, represented as 1 dimensional spheres (top right) and measure the inner products on each of them independently (bottom right), we can efficiently detect  the symmetries underlying the point distribution on the sphere and distinguish that the points lie on two different great circles.}
    \label{fig:subspace}
\end{figure}
Moreover, suppose the embedding function $E$ is trained end-to-end. In that case, the independent subspaces allow the embedder to specialize each subspace on different data characteristics, enabling the measurement of similarities on distinct data features.
\marco{Sarebbe bello mettere un toy example che fa vedere come questa divisione in sottospazi sia utile a distinguere casi che  vogliamo distinguere, o ad essere invarianti. In maniera simile rispetto agli esempi dell'isometria e della quasi isometria. Forse ne ho in mente uno } \luca{Yes sembra perfetto! Dici aggiungiamo direttamente qui l'esempio?}



\subsection{Subspace comparison}\label{sec:subspace-comparison}
In this section, we demonstrate the effectivness of the subspace strategy described \Cref{sec:subspaces}. 

\paragraph{Experimental setting.} We consider the classification and reconstruction tasks on the \mnist{} and \cifart{}. The models compared a classifier and autoencoder that employs the relative representation with an increasing number of subspaces.

The results reported in \Cref{tab:subspace-performance-comparison} show that subdiving the latent space in multiple subspaces improves the expressivness of the architecture and the performance on classification and reconstruction tasks.

\begin{table}[ht]
\caption{\draft{TBA} Performance comparison between different number of subspaces subdivision.}
\label{tab:subspace-performance-comparison}
\begin{center}
\begin{tabular}{ccccccc|cccccc}
& \multicolumn{6}{c}{\bf Classification }  & \multicolumn{6}{c}{\bf Reconstruction} \\
Subspaces & $1$ &  $2$ &  $4$ &  $8$ &  $16$ &  $32$ & $1$ &  $2$ &  $4$ &  $8$ &  $16$ &  $32$ \\ 
\\ \hline \\
\mnist{} & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?  \\
\cifart{} & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?  \\
\end{tabular}
\end{center}
\end{table}


\subsection{Interpretability}\label{sec:interpretability}
The similarity function infuses specific properties in the latent representation. In this work, our focus has been on the cosine similarity that induces an isometry invariant representation.
This section contains an example of an alternative similarity function, that besides the isometry invariance, infuses other properties in the latent representation.

\textbf{Experimental setting.}
We define two \glspl{ae} that utilize the relative representations in the bottleneck. The first \gls{ae} adopts the cosine similarity as described in \Cref{sec:isometry-invariance}; the second \gls{ae} performs a change of basis solving the following linear system $\ve_{\sA} \vr_{\vx^{(i)}} = \ve_{\vx^{(i)}}$. That is, we represent the absolute embedding $\ve_{\vx^{(i)}}$ of a sample $\vx^{(i)}$ as the coefficients of the basis formed by the embeddings $\ve_{\sA}$ of all the anchors $\sA$. We train both \glspl{ae} end-to-end on the \mnist{} dataset.

The basis-change method forces the anchors to be a basis for the relative latent space, thus a higher similarity value on the $i$ dimension indicates a higher coefficient for the $i$-th anchor. In \Cref{fig:interpretability} we compare the reconstructions performed by decoders trained with relative representations obtained with the cosine similarity (bottom row) and the basis-change method (top row). The relative representations provided are zero everywhere except that in one dimension. When adopting the basis-change strategy, the reconstructed images are similar to the anchor associated with the non-zero dimension.
Since the anchors $\va^{(j)}$ have intelligible also the corresponding dimension in the relative representation $\vr_{j}$ becomes interpretable.

\begin{figure}[ht]
    \centering
    \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=1\linewidth]{figures/mockup/interpretability.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
        %
    \end{overpic}
    \vspace{-.5cm}
    \caption{\draft{TBA} Relative representation properties comparison. Each image is a reconstruction given the relative representation shown on its left. The relative representation shows the anchors associated with each dimension, it is zero in all dimensions except one. The images in the top row are obtained with a decoder trained with the basis change as similarity measure; the bottom row images are produced by a decoder trained with the cosine similarity. }
    \label{fig:interpretability}
\end{figure}


\subsection{Word Analogies}\label{sec:analogies}
Possibile esperimento 1 per validare questa cosa: testiamo il benchmark base di word analogies (e simili, molto semplice/immediato) sia con encoding assoluto che relativo (stessa lingua). Se il relativo va meglio: siamo piu' astratti. Se l'assoluto va meglio: non si mette l'esperimento (tanto c'e' la citazione a https://www.frontiersin.org/articles/10.3389/frai.2021.698809/full) .
Consideriamo il task di calcolare la distanza fra coppie di parole
Il gold standard contro cui testarsi è annotazionie umana
We evaluate the correlations between the gold standard distances and the distances predicted by the model
Prendiamo gli embedding fasttext
In this setting we do not train any neural network, but we evaluate the goodness of the word representation

\begin{table}[ht]
\caption{\luca{WIP}  
}
\label{tab:word-analogies}
\begin{center}
\begin{tabular}{lccc}
\multicolumn{1}{c}{ \bf Embedding Type} & 
\multicolumn{1}{c}{ \bf  Score } & 
\\[.5ex] \hline \\
Relative FastText & ?  & ?  & ?          \\               
Absolute FastText  & ? & ? & ?          \\          
\end{tabular}
\end{center}
\end{table}


\subsubsection{Cross-domain stitching}\label{sec:model-reusability-domain}
In this section we demonstrate relative representations generate compatible latent spaces even \emph{across different data domains}, as long as the data represents the same information and there are parallel anchors in correspondence between the domains. 

\paragraph{Experimental setting.} We consider a classification task on the datasets: 
\thingi{}   \cite{Zhou_undated-jc},
\surreal{}  \cite{Varol2017-et},
\deformingthings{} \cite{Li2021-yv}, \shapenet{}. Note that these datasets contains the 3D model of each object associated with the corresponding 2D rendering.
We define two encoders: 
one to embed images $E^{RGB}$ 
and one to embed points clouds  $E^{PC}$. 
Thus, we choose image-3D parallel anchors that allow to define relative representation between the embeddings of images and between the embeddings of point clouds. 
Furthermore, we define a neural component $D$ that takes a  representation and predicts the object category.
We performs experiments to showcase the resulting alignment of the relative representations in the two domains and the zero-shot cross-domain capabilities, switching encoder without re-training or fine-tuning the classifier component. 

The results in \Cref{tab:cross-domain} prove that the absolute representation completely fail when performing zero-shot cross-domain classification. Meanwhile, the relative representation demonstrate a certain degree of compatibility between the latent spaces of images and point clouds.

\begin{table}[ht]
\caption{\draft{TBA} Cross-domain performance comparison. Each column is trained on the indicated dataset with the reported encoder, thus the resulting classifier component $D$ is stitched together with the encoder reported on each row to perform zero-shot classification. The row also indicates whether the relative representations are employed or not. The numbers reported are the accuracy on the test set of each dataset. }
\label{tab:cross-domain}
\begin{center}
\begin{tabular}{cllllllllll}
& & & \multicolumn{8}{c}{\bf Training }  \\
& & & \multicolumn{2}{c}{\thingi{} }  
& \multicolumn{2}{c}{\surreal{} }  
& \multicolumn{2}{c}{\deformingthings{} }  
& \multicolumn{2}{c}{\shapenet{} } \\[.5ex]
& & & $E^{RGB}$ & $E^{PC}$
& $E^{RGB}$ & $E^{PC}$
& $E^{RGB}$ & $E^{PC}$
& $E^{RGB}$ & $E^{PC}$ 
 \\ \hline \\ 
\multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\bf Stitching}}} & \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{Rel.}}} & $E^{RGB}$ & ? & ? & ?  & ? & ? & ? & ?  & ? \\
& & $E^{PC}$ & ? & ? & ?  & ? & ? & ? & ?  & ? \\[1ex]
&  \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{Abs.}}} & $E^{RGB}$ & ? & ? & ?  & ? & ? & ? & ?  & ? \\
& & $E^{PC}$ & ? & ? & ?  & ? & ? & ? & ?  & ? \\
\end{tabular}
\end{center}
\end{table}



\subsection{Self-representation computation}

 \begin{figure}[!h]
    \centering
    \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=.5\linewidth]{figures/mockup/method.pdf}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
    \end{overpic}
    \caption{\draft{TBA} \luca{Change image symbol} Relative representation computation: 
    (1) the function $E$ embeds the sample $x^{(i)}$; 
    (2) the function $E$ embeds all the anchors $a^{(1)}, \dots, a^{(|\sA|)}$; 
    (3) the similarities between the sample embedding and anchors embeddings are the relative representation of the sample.}
    \label{fig:method}
\end{figure}

% Cross-archtecture
% Osservazione iniziale: se rappresentiamo una parola grazie alle relazioni/distanze che ha con altre parole, allora stiamo implicitamente passando ad una rappresentazione di piu' alto livello (circa concetti, anche se restano ambigue). Poiche' all'interno dell'embedding relativo stesso c'è l'infromazione di come si dispone quella rispetto tutte le altre (ancore).
%
% Luca: Move somewhere else: 
% Relative representations can be applied in the distributional semantics context, where the so called "semantic horizon" of a word (and more in general, a concept) can easily be described by looking at its neighborhood. In fact, most of the relations in semantic spaces are \textit{local}, meaning that to describe a concept it is more useful to have information about the region of the space surrounding it than about the whole structure of the space in which it is embedded. By transposing this property in our setting, we can show how the relative representations of words gain in abstraction power, enabling a swap between language specific encoders by construction.

\subsection{Robustness Analysis}\label{sec:quantization-performance}
 
\begin{figure}[ht]
    \centering
    \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=.7\linewidth]{figures/mockup/marco-quantization.png}
        %  trim={<left> <lower> <right> <upper>}
        %  \put(horiz, vert)
        %  \put(horiz, vert){\rotatebox{90}{Text}}
    \end{overpic}
    \caption{\draft{TBA} Reconstruction errors on the \cifart{} dataset at different quantization bin sizes. The models shown are: $RAE^b_{E_1D_1}$ quantized and trained end-to-end, $RAE_{E_1D_1}$ non-quantized and trained end-to-end, $RAE^b_{E_1D_2}$ quantized and stitched together, $RAE_{E_1D_2}$ non-quantized and stitched together. The quantization improves the robustness of the models stitched together since enhances the latent space isometry invariance.}
    \label{fig:quantization-performance}
\end{figure}

